LDPC Decoding with Degree-Specific Neural Message Weights and RCQ Decoding

Recently, neural networks have improved MinSum message-passing decoders for low-density parity-check (LDPC) codes by multiplying or adding weights to the messages, where the weights are determined by a neural network. The neural network complexity to determine distinct weights for each edge is high, often limiting the application to relatively short LDPC codes. Furthermore, storing separate weights for every edge and every iteration can be a burden for hardware implementations. To reduce neural network complexity and storage requirements, this paper proposes a family of weight-sharing schemes that use the same weight for edges that have the same check node degree and/or variable node degree. Our simulation results show that node-degree-based weight-sharing can deliver the same performance requiring distinct weights for each node. This paper also combines these degree-specific neural weights with a reconstruction-computation-quantization (RCQ) decoder to produce a weighted RCQ (W-RCQ) decoder. The W-RCQ decoder with node-degree-based weight sharing has a reduced hardware requirement compared with the original RCQ decoder. As an additional contribution, this paper identifies and resolves a gradient explosion issue that can arise when training neural LDPC decoders.

==> 8k_configuration.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption {The Quantizer/Dequantizer pairs of W-OMS-RCQ decoder for (9472,8192) LDPC code}
\label{tab: 8k_config}
\begin{tabular}{|c|c|c|}
\hline
 CN bitwidth             & Quantizer/Reconstruction Parameter & Corresponding Decoder Iteration \\ \hline
4 bits                  & $C=7$, $\gamma=1.7$                                                                       & $1\sim10$                                                                        \\ \hline
\multirow{3}{*}{3 bits} & $C_1=3$, $\gamma_1=1.3$                                                                     & $1\sim6$                                                                         \\ \cline{2-3} 
                        & $C_2=5$, $\gamma_2=1.3$                                                                    & $7\sim8$                                                                         \\ \cline{2-3} 
                        & $C_3=7$, $\gamma_3=1.3$                                                                      & $9\sim10$                                                                        \\ \hline
\end{tabular}
\end{table}

==> memory_optimization.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tp]
\caption {Memory requirement for storing messages of MS decoder} \label{tab: memory_requirement} 
\centering
\begin{tabular}{|c|c|c|c|}
\hline
                                                                                & Variables                                 & Data type     & Required amount \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Before \\ optimization\end{tabular}} & $l_{v\rightarrow c}^{(t)}$                & double 64-bit & $EI_T$          \\ \cline{2-4} 
                                                                                & $u_{c\rightarrow v}^{(t)}$                & double 64-bit & $EI_T$          \\ \cline{2-4} 
                                                                                & $l_v^{(t)}$                               & double 64-bit & $nI_T$          \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}After \\ optimization\end{tabular}}  & $\texttt{min1}_c^{(t)}$                   & double 64-bit & $(n-k)I_T$      \\ \cline{2-4} 
                                                                                & $\texttt{pos1}_c^{(t)}$                   & int 32-bit    & $(n-k)I_T$      \\ \cline{2-4} 
                                                                                & $\texttt{min2}_c^{(t)}$                   & double 64-bit & $(n-k)I_T$      \\ \cline{2-4} 
                                                                                & $\texttt{pos2}_c^{(t)}$                   & int 32-bit    & $(n-k)I_T$      \\ \cline{2-4} 
                                                                                & \text{sgn}$\left(u_{c\rightarrow v}\right)$ & bool 1-bit    & $EI_T$          \\ \cline{2-4} 
                                                                                & \text{sgn}$\left(l_{v\rightarrow c}\right)$ & bool 1-bit    & $EI_T$          \\ \hline
\end{tabular}
\end{table}

==> weight_sharing.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[t]
\centering
\caption{Various Node-Degree-Based Weight Sharing Schemes and\\ Required Number of Parameters per Iteration for Two Example Codes}
\begin{tabular}{|m{5mm}c|c|c|c|c|}
\hline
\multirow{2}{*}{Type} & \multirow{2}{*}{$\beta^{(t)}_{*}$}                                    & \multirow{2}{*}{$\alpha^{(t)}_{*}$}                & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}The Number of Required\\  Parameters per Iteration\end{tabular}}                        \\ \cline{4-5} 
                      &                                                                       &                                                    & (16200,7200) DVBS-2 code & (3096,1032)  PBRL code \\ \hline
\multicolumn{5}{|c|}{No Weight Sharing\cite{Nachmani2016-bs}}                                                                                                                                                                                                                                                     \\ \hline
$0$            & $\beta^{(t)}_{(c_i,v_j)}$                                             & 1                                                  & $4.8*10^5$                                                          & $1.60*10^4$                                                      \\ \hline
\multicolumn{5}{|c|}{Weight Sharing Based on Node Degree}                                                                                                                                                                                                                                   \\ \hline
1                     & $\beta^{(t)}_{(\text{deg}{(c_i)},\text{deg}{(v_j)})}$                                 & 1                                                  & 13                                                                  & 41                                                               \\ \hline
2                     & $\beta^{(t)}_{(\text{deg}{(c_i)})}$                                          & $\alpha^{(t)}_{(\text{deg}{(v_j)})}$                      & 8                                                                   & 15                                                               \\ \hline
3                     & $\beta^{(t)}_{(\text{deg}{(c_i)})}$                                          & 1                                                  & 4                                                                   & 8                                                                \\ \hline
4                     & 1                                                                  & $\alpha^{(t)}_{(\text{deg}{(v_j)})}$                      & 4                                                                   & 7                                                                \\ \hline
\multicolumn{5}{|c|}{Weight Sharing Based on Protomatrix}                                                                                                                                                                                                                                   \\ \hline
5\cite{dai2021learning}          & $\beta^{(t)}_{\left( \floor{\frac{i}{f}},\floor{\frac{j}{f}}\right)}$ & 1                                                  & $-$                                                                 & 101                                                              \\ \hline
6                     & $\beta^{(t)}_{\left( \floor{\frac{i}{f}}\right)}$                     & 1                                                  & $-$                                                                 & 17                                                               \\ \hline
7                     & 1                                                                       & $\alpha^{(t)}_{\left( \floor{\frac{j}{f}}\right)}$ & $-$                                                                 & 25                                                               \\ \hline
\multicolumn{5}{|c|}{Weight sharing based on Iteration  \cite {Lian2019-jh,Abotabl2019-wt}}                                                                                                                                                                                                          \\ \hline
8                     & $\beta^{(t)}$                                                         & 1                                                  & 1                                                                   & 1                                                                \\ \hline
\end{tabular}\label{tab:weight_sharing}
\end{table}
